The Importance of Worst-Case Memory Contention Analysis for Heterogeneous SoCs

Memory interference may heavily inflate task execution times in Heterogeneous Systems-on-Chips (HeSoCs). Knowing worst-case interference is consequently fundamental for supporting the correct execution of time-sensitive applications. In most of the literature, worst-case interference is assumed to be generated by, and therefore is estimated through read-intensive synthetic workloads with no caching. Yet these workloads do not always generate worst-case interference. This is the consequence of the general results reported in this work. By testing on multiple architectures, we determined that the highest interference generation traffic pattern is actually hardware dependant, and that making assumptions could lead to a severe underestimation of the worst-case (in our case, of more than 9x).

==> sections/experiments.tex <==
\section{Last-Level Cache Eviction}
\label{sec:exp}
Understanding why some real benchmarks suffer more interference than the synthetic ones requires further investigation.
Interference analysis works under the assumption that the sole motivation for delayed execution time is resource contention along the path between the L2 cache and the DRAM controller.
Under this assumption, we don't expect the number of transactions along this path (i.e., the number of cache misses) to increase.

To shed some light, we thus extend our experimental setup with the capability of measuring such number of transactions using the Performance Monitoring Units (PMUs), and specifically the hardware counter \texttt{L2D\_CACHE\_REFILL}. In our next experiment, we use our synthetic benchmark as a \textit{task under test}, and we vary their memory footprint ($f\!p$).
%
As interference tasks we use the \textit{READ\_MISS} benchmark, with $f\!p$ = 512KB.

Considering that the size of the L2 cache is 1MB, for the \textit{task under test} we make use of two settings for $f\!p$ that are below this value and two values that are above.
When $f\!p$ is larger than the L2 cache, the benchmarks always generate 100\% L2-cache refills, regardless of the \textbf{THR\%} setting used for the \textit{interference tasks}.
This is clearly visible in Fig. \ref{fig:LASTd}, where the curves are completely flat.
This however is not reflected in the timing behavior in Fig. \ref{fig:LASTa}, where the green and purple lines grow beyond\textbf{ THR\%} = 20\%.

When $f\!p$ is smaller than the L2 cache, the benchmark itself generates 0\% L2 cache miss (besides cold cache misses), but as \textbf{THR\%} grows we start observing an increasing number of L2 cache refill events.
This is due to the fact that the interference tasks are heavily modifying the content of L2 as they execute, continuously evicting relevant data to the task under test.
This thrashing effect is responsible for the increase in execution time that we observe in Fig. \ref{fig:LASTa} for the red and blue curves up until \textbf{THR\%}.
Beyond that point, the phenomenon is the same that we discussed for larger $f\!p$ than the L2 cache.

To demonstrate that these newly discovered effects are responsible for the higher than expected interference experienced by the Polybench benchmarks (ABOVE adn ACROSS red and yellow areas) in Figg. \ref{fig:interf_NVIDIA} and \ref{fig:interf_XILINX}, when READ\_MISS is the interfering task, we compare the execution time results reported there with the L2 cache activity.
Specifically, we introduce the following metric:
%
\begin{equation}
    RF_{THR_x} = \frac{refill_{THR_x}}{refill_{THR_0}}\times\frac{refill_{THR_x}}{MEM\_ACCESS}
    \label{eqn:refill-metric}
\end{equation}
%

The first term of this equation represents the the increase in refills due to L2 cache \textit{thrashing} by the \textit{interference tasks}.
%represented by the term $refill_{THR_x}$, this value is normalized by the number of refills when no other programs are running on the platform ($refill_{THR_0}$). 
The second term represents the overall L2 cache miss rate induces by such refills\footnote{The impact of a high refill increase is still low if the cache miss rate is low.}.
% However, this first term alone is not sufficient to explain the actual behaviour of the increase in execution time, unlike the synthetic workloads discussed above. This because a significant increase in refills could not reflect on the execution time, if the percentage of refills, respect to the whole memory accesses is low. To retrieve this information we leveraged the \texttt{MEM\_ACCESS} performance counter, a raw counting on the total memory accesses performed by the application.
% These aspects are quantified by the second term of the equation. The $RF$ metric applied to the PolyBench is reported in Fig. \ref{fig:nvidia-polybench-second} and \ref{fig:xilinx-polybench-second}. Here it is important to remark two fundamental aspects: i) the applications that are less subject to last-level cache thrashing are characterized by an almost horizontal $RF$ curve (this is the case of the \texttt{READ\_MISS} application); ii) the higher is the $RF$ metric the higher is the impact on execution time (we expect a high $RF$ for the benchmarks that belong to Region 1).

Figg. \ref{LAST:b} and \ref{LAST:e} show the results for the NVIDIA SoC, whereas Figg. \ref{LAST:c} and \ref{LAST:f} show the results for the XILINX SoC.
It is possible to see that the synthetic benchmarks have flat RF curves (subplots \textit{e} and \textit{f}), indicating that they are not subject to the L2 cache \textit{thrashing} phenomenon.
The increase in execution time that they experience is thus only due to proper resource contention along the L2-to-DRAM path.
On the contrary, the shape of the red and yellow areas in subplots \textit{e} and \textit{b} for NVIDIA and in subplots \textit{f} and \textit{f} for XILINX demonstrates that the culprit for execution time increase in the Polybench benchmarks is L2 cache behavior under interference.
